PipeRAG: Fast Retrieval-Augmented Generation via Algorithm-System Co-design

Retrieval-augmented generation (RAG) can enhance the generation quality of large language models (LLMs) by incorporating external token databases. However, retrievals from large databases can constitute a substantial portion of the overall generation time, particularly when retrievals are periodically performed to align the retrieved content with the latest states of generation. In this paper, we introduce PipeRAG, a novel algorithm-system co-design approach to reduce generation latency and enhance generation quality. PipeRAG integrates (1) pipeline parallelism to enable concurrent retrieval and generation processes, (2) flexible retrieval intervals to maximize the efficiency of pipeline parallelism, and (3) a performance model to automatically balance retrieval quality and latency based on the generation states and underlying hardware. Our evaluation shows that, by combining the three aforementioned methods, PipeRAG achieves up to 2.6$\times$ speedup in end-to-end generation latency while improving generation quality. These promising results showcase the effectiveness of co-designing algorithms with underlying systems, paving the way for the adoption of PipeRAG in future RAG systems.

==> motivation.tex <==
\section{Motivation: Improve RAG Efficiency}
\label{sec:motivation}

Although periodically retrieving tokens from a large database can effectively improve the generation quality of LLMs, the frequent retrievals can account for a considerable portion of the total generation time, thereby slowing down the end-to-end generation process.


In this paper, we ask the following question: \textbf{is it possible to further enhance the efficiency of retrieval augmented generation?} Here, we conceptualize \textit{RAG efficiency} as a Pareto frontier considering two objectives: \textit{generation quality} and \textit{system performance}. 
Specifically, given a quality requirement (achieving certain perplexity), can we optimize RAG's system performance (reducing generation latency)? On the other hand, given a system performance requirement, can we improve the quality of generation? 


% The goal of this paper, i.e., efficient machine learning, is shared by other widely-adopted machine learning techniques such as model quantization and pruning: by downgrading the numerical precision used in computations. By representing weights and activation with fewer bits, quantization can notably decrease the memory footprint and accelerate inference without significantly impacting model performance. Another method is sparsity, which capitalizes on the fact that many parameters in a neural network are often minimal and contribute little to the output. Pruning these negligible weights results in a sparse model that is more efficient in terms of storage and computation. 

% Additionally, distributed machine learning strategies, such as asynchronous updates, facilitate training over extensive datasets by distributing the workload across multiple machines or processors. This method allows for training without requiring synchronization at every step, enhancing speed and scalability.

% Applying the principles of efficient machine learning to Retrieval-Augmented Generation (RAG) reveals a key inefficiency: the dependency between language generation and retrieval. Firstly, given that RAG's advantage is a smaller LLM coupled with a large knowledge database achieving comparable or better quality than a larger LLM, retrieval latency becomes a significant portion of the total generation latency. Secondly, as indicated in Figure~\ref{}, either the LLM generation system or the vector retrieval system is idle at any given point during inference, leading to a low utilization rate. It's generally impractical to combine these two systems on the same hardware platform. If both are on CPUs, LLM inference is significantly slower without GPU acceleration. Moreover, with a large retrieval database (e.g., billions of vectors), it's unfeasible to house the database on a single GPU due to capacity constraints. Transferring vectors from the GPU's host CPU server would further slow down retrieval performance compared to CPU usage, due to limited bandwidth between CPU and GPU.

% In this paper, we explore whether it's possible to optimize RAG performance (e.g., latency) by breaking this dependency chain and thereby maximizing hardware resource utilization. To this end, we introduce PipeRAG as follows.

